Diffusion-Guided Reconstruction of Everyday Hand-Object Interaction Clips

We tackle the task of reconstructing hand-object interactions from short video clips. Given an input video, our approach casts 3D inference as a per-video optimization and recovers a neural 3D representation of the object shape, as well as the time-varying motion and hand articulation. While the input video naturally provides some multi-view cues to guide 3D inference, these are insufficient on their own due to occlusions and limited viewpoint variations. To obtain accurate 3D, we augment the multi-view signals with generic data-driven priors to guide reconstruction. Specifically, we learn a diffusion network to model the conditional distribution of (geometric) renderings of objects conditioned on hand configuration and category label, and leverage it as a prior to guide the novel-view renderings of the reconstructed scene. We empirically evaluate our approach on egocentric videos across 6 object categories, and observe significant improvements over prior single-view and multi-view methods. Finally, we demonstrate our system's ability to reconstruct arbitrary clips from YouTube, showing both 1st and 3rd person interactions.

==> exp/ablate_anneal.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{exp/anneal.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}



==> exp/more_frame.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{exp/more_frame.pdf}
    \caption{More frame helps \todo{less training/try no RGB} ? }
    \label{fig:my_label}
\end{figure}

==> exp/table2.tex <==


%------------------------------------------------------------------------

% \definecolor{first}{rgb}{1.0, .79, 0.156}
\definecolor{first}{rgb}{1.0, .83, 0.3}
\definecolor{second}{rgb}{1.0, 0.93, 0.7}
% \definecolor{second}{rgb}{1.0, 0.88, 0.51}
% \definecolor{third}{rgb}{1.0, 0.93, 0.7}
\def \first {\cellcolor{first}}
\def \second {\cellcolor{second}}
% \def \third {\cellcolor{third}}
\def \third {}


\begin{table*}[t]
\footnotesize
\begin{center}
% \vspace{1em}
% \caption{\textbf{Comparison of F1@5mm, F1@10mm scores and Chamfer distance:} Ablation with no prior, hand prior and object prior}

\caption{\textbf{Analysis of category and HOI prior effects on object reconstruction:} Quantitative results for object reconstruction error using F1@5mm and F1@10mm scores and Chamfer Distance (mm). We compare our method  with ablations that consider no prior,  category prior only, and hand prior only on the HOI4D dataset.}
\label{tab:prior_obj}

% \vspace{-1em}
\setlength{\tabcolsep}{2pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l ccc ccc ccc ccc ccc ccc ccc}
\toprule


% CATEGORIES
& \multicolumn{3}{c}{Mug} 
& \multicolumn{3}{c}{Bottle}
& \multicolumn{3}{c}{Kettle} 
& \multicolumn{3}{c}{Bowl} 
& \multicolumn{3}{c}{Knife} 
& \multicolumn{3}{c}{ToyCar} 
& \multicolumn{3}{c}{Mean}\\

% RULES
\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} \cmidrule(r){11-13} \cmidrule(r){14-16}
\cmidrule(r){17-19} \cmidrule(r){20-22}

% PSNR LPIPS LABELS
& $F@5$  & $F@10$ & $CD$  
& $F@5$  & $F@10$ & $CD$  
& $F@5$  & $F@10$ & $CD$  
& $F@5$  & $F@10$ & $CD$  
& $F@5$  & $F@10$ & $CD$  
& $F@5$  & $F@10$ & $CD$  
& $F@5$  & $F@10$ & $CD$  
\\


% NUMBERS
\midrule
no-prior & 0.46 & 0.73 & 1.8 & 0.39 & 0.65 & 2.2 & 0.18 & 0.39 & 9.1 & \second 0.45 & \second 0.73 & \second 1.9 & \first \textbf{0.70} & 0.93 & \first \textbf{0.5} & 0.63 & 0.92 & 0.6 & 0.47 & 0.73 & 2.7 \\
hand-prior & 0.48 & 0.77 & 1.4 & 0.37 & 0.66 & 1.6 & 0.30 & 0.60 & 3.4 & 0.38 & 0.63 & 4.2 & 0.09 & 0.24 & 5.8 & 0.70 & 0.97 & 0.4 & 0.39 & 0.65 & 2.8 \\
cat-prior & \second 0.62 & \second 0.85 & \second 1.1 & \first \textbf{0.56} & \first \textbf{0.95} & \first \textbf{0.6} & \first \textbf{0.63} & \first \textbf{0.94} & \first \textbf{0.7} & 0.35 & 0.58 & 5.8 & 0.44 & \second 0.94 & 0.8 & \second 0.77 & \second 0.98 & \second 0.4 & \second 0.56 & \second 0.87 & \second 1.6 \\
Ours & \first \textbf{0.64} & \first \textbf{0.86} & \first \textbf{1.0} & \second 0.54 & \second 0.92 & \second 0.7 & \second 0.43 & \second 0.77 & \second 1.5 & \first \textbf{0.79} & \first \textbf{0.98} & \first \textbf{0.4} & \second 0.50 & \first \textbf{0.95} & \second 0.8 & \first \textbf{0.83} & \first \textbf{0.99} & \first \textbf{0.3} & \first \textbf{0.62} & \first \textbf{0.91} & \first \textbf{0.8} \\

% no prior & 0.39 & 0.66 & 2.2 & 0.39 & 0.63 & 2.3 & 0.15 & 0.35 & 11.6 & \second 0.41 & \second 0.70 & \second 2.1 & \second 0.70 & 0.93 & \second 0.5 & 0.66 & 0.92 & 0.6 & 0.45 & 0.70 & 3.22 \\

% hand prior & 0.52 & 0.78 & 1.4 & 0.36 & 0.63 & \second 1.8 & 0.13 & 0.29 & 6.3 & 0.35 & 0.57 & 5.5 & 0.57 & \second 0.96 & 0.6 & \second 0.73 & \second 0.98 & \first \textbf{0.4} & 0.44 & 0.70 & 2.65 \\

% category prior & \second 0.62 & \second 0.87 & \second 0.9 & \second 0.43 & \second 0.71 & 2.9 & \second 0.65 & \first \textbf{0.89} & \first \textbf{1.0} & 0.26 & 0.43 & 9.2 & 0.46 & 0.95 & 0.8 & 0.70 & \first \textbf{0.98} & \second 0.4 & \second 0.52 & \second 0.81 & \second 2.53 \\

% Ours & \first \textbf{0.66} & \first \textbf{0.89} & \first \textbf{0.8} & \first \textbf{0.84} & \first \textbf{0.99} & \first \textbf{0.3} & \first \textbf{0.71} & \second 0.88 & \second 1.1 & \first \textbf{0.50} & \first \textbf{0.86} & \first \textbf{0.9} & \first \textbf{0.74} & \first \textbf{0.98} & \first \textbf{0.4} & \first \textbf{0.75} & 0.97 & 0.4 & \first \textbf{0.70} & \first \textbf{0.93} & \first \textbf{0.66} \\

\bottomrule
\vspace{-3.5em}
\end{tabular}
}

\end{center}

\end{table*}
% \vspace{-5em}

==> exp/table3.tex <==


%------------------------------------------------------------------------

% \definecolor{first}{rgb}{1.0, .79, 0.156}
\definecolor{first}{rgb}{1.0, .83, 0.3}
\definecolor{second}{rgb}{1.0, 0.93, 0.7}
% \definecolor{second}{rgb}{1.0, 0.88, 0.51}
% \definecolor{third}{rgb}{1.0, 0.93, 0.7}
\def \first {\cellcolor{first}}
\def \second {\cellcolor{second}}
% \def \third {\cellcolor{third}}
\def \third {}


\begin{table}[t!]
\footnotesize
\begin{center}
% \vspace{1em}
% \caption{\textbf{Analysis of category and HOI prior ablations on alignment between hands and objects:} We compare the Chamfer Ablation with no prior, hand prior and object prior \yy{@ poorvi -- can you add a middle rule under no prior and highlight the top 1 results of (hand prior, object prior and ours)? and make the tables in uniform font size}}

\caption{\textbf{Analysis of category and HOI prior effects on hand-object relation:} Quantitative results for hand-object alignment using Chamfer distance (mm) in hand frame ($\text{CD}_{\text{h}}$). We compare our method with ablations that only incorporate the category prior, the hand prior, and no prior on the HOI4D dataset. The highlighted results are only compared among with-prior variants as the no-prior variant does not generate realistic shapes shown in Fig.~\ref{fig:prior} thus not comparable. } 
\label{tab:prior_hand}



% \vspace{-1em}
\setlength{\tabcolsep}{2pt}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l c c c c c c c}
\toprule


% CATEGORIES
& \multicolumn{1}{c}{Mug} 
& \multicolumn{1}{c}{Bottle}
& \multicolumn{1}{c}{Kettle} 
& \multicolumn{1}{c}{Bowl} 
& \multicolumn{1}{c}{Knife} 
& \multicolumn{1}{c}{ToyCar} 
& \multicolumn{1}{c}{Mean}\\

% RULES
% \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} \cmidrule(r){11-13} \cmidrule(r){14-16}
% \cmidrule(r){17-19} \cmidrule(r){20-22}

% PSNR LPIPS LABELS
% & $F@5$  & $F@10$ & $CD$  
% & $F@5$  & $F@10$ & $CD$  
% & $F@5$  & $F@10$ & $CD$  
% & $F@5$  & $F@10$ & $CD$  
% & $F@5$  & $F@10$ & $CD$  
% & $F@5$  & $F@10$ & $CD$  
% & $F@5$  & $F@10$ & $CD$  
% \\


% NUMBERS
\midrule
no-prior & 36.0 & 15.4 & 58.2 & 75.7 & 29.5 & 7.1 & 37.0 \\
\midrule
hand-prior & 34.5 & \second 18.3 & 57.5 & \first \textbf{87.5} & \first \textbf{71.7} & 60.6 & \second 55.0 \\
cat-prior & \second 23.2 & 75.7 & \second 54.4 & 158.6 & 164.0 & \second 34.9 & 85.2 \\
Ours & \first \textbf{18.1} & \first \textbf{15.3} & \first \textbf{42.2} & \second 101.8 & \second 82.9 & \first \textbf{23.3} & \first \textbf{47.2} \\

% no prior & 44.2 & 8.5 & 51.4 & 39.7 & 35.3 & 5.9 & 30.83 \\
% \midrule
% hand prior & 27.3 & \second 15.0 & \second 52.0 & \first \textbf{78.3} & \first \textbf{45.5} & 51.5 & \second 44.94 \\

% category prior & \second 26.1 & 31.8 & 53.6 & 129.2 & 86.4 & \second 43.8 & 61.82 \\

% Ours & \first \textbf{20.4} & \first \textbf{12.2} & \first \textbf{45.2} & \second 92.8 & \second 53.8 & \first \textbf{27.0} & \first \textbf{41.92} \\

\bottomrule
\vspace{-3.5em}
\end{tabular}
}

\end{center}

\end{table}
% \vspace{-5em}

